Embedding Cultural Diversity in Prototype-based Recommender Systems

Popularity bias in recommender systems can increase cultural overrepresentation by favoring norms from dominant cultures and marginalizing underrepresented groups. This issue is critical for platforms offering cultural products, as they influence consumption patterns and human perceptions. In this work, we address popularity bias by identifying demographic biases within prototype-based matrix factorization methods. Using the country of origin as a proxy for cultural identity, we link this demographic attribute to popularity bias by refining the embedding space learning process. First, we propose filtering out irrelevant prototypes to improve representativity. Second, we introduce a regularization technique to enforce a uniform distribution of prototypes within the embedding space. Across four datasets, our results demonstrate a 27\% reduction in the average rank of long-tail items and a 2\% reduction in the average rank of items from underrepresented countries. Additionally, our model achieves a 2\% improvement in HitRatio@10 compared to the state-of-the-art, highlighting that fairness is enhanced without compromising recommendation quality. Moreover, the distribution of prototypes leads to more inclusive explanations by better aligning items with diverse prototypes.

==> figure_texs/prototype_distances.tex <==
 \begin{figure}[h]
  \centering
  \includegraphics[scale=0.45]{figs/distances.png} 
  \caption{Average cosine distance to k-nearest prototypes across items with different popularity levels. The ProtoMF model is trained on the LastFM-2b dataset with 80 prototypes.} 
  \label{fig:prototype_distances}
\end{figure}


==> tables/different_settings_LastFM.tex <==
\begin{table}[h]
    \centering
    \caption{Performance and Fairness of ProtoMF on the LastFM-2b Dataset Across Different Combinations of $k$ (Prototype Filtering) and $\lambda$ (Regularization Strength), where  $k=-1$ indicates using all prototypes.}
    \label{tab:all_experiment_results}
    \begin{tabular}{c|c|c|c|c|c}
        \toprule
        \( K_u \) & \( \lambda_u \) & \( K_t \) & \( \lambda_t \) & HitRatio@10 & NDCG@10  \\
        \midrule
        
        -1 & 0.0 & 60 & 0.0 & 0.593 & 0.348\\ 
        \hline
                
        60 & 0.003 & 60 & 0.1 & 0.577 & 0.338 \\ 
        \hline
                
        60 & 0.0 & 25 & 0.003 & 0.569 & 0.332 \\ 
        \hline
                
        -1 & 0.0 & 25 & 0.003 & 0.569 & 0.329 \\ 
        \hline
                
        -1 & 0.0 & 60 & 0.9 & 0.562 & 0.326 \\ 
        \hline
                
        -1 & 0.0 & 40 & 0.0 & 0.559 & 0.321 \\ 
        \hline
                
        12 & 1.0 & 12 & 0.1 & 0.552 & 0.323 \\ 
        \hline
                
        -1 & 0.0 & 60 & 0.25 & 0.552 & 0.320 \\ 
        \hline
                
        -1 & 0.0 & 12 & 0.0 & 0.543 & 0.310 \\ 
        \hline

                
        -1 & 0.0 & 60 & 0.387 & 0.534 & 0.307 \\ 
        \hline

                
        -1 & 0.1 & 25 & 0.0 & 0.519 & 0.301 \\ 
        \hline

                
        60 & 0.003 & 60 & 0.003 & 0.515 & 0.301 \\ 
        \hline

                
        25 & 0.0 & 25 & 10.0 & 0.513 & 0.294 \\ 
        \hline

                
        -1 & 10.0 & 40 & 40 & 0.505 & 0.291 \\ 
        \hline

                
        -1 & 0.0 & 12 & 0.0 & 0.488 & 0.273 \\ 
        \hline
        
        
        
        \bottomrule
    \end{tabular}
\end{table}

==> tables/distances.tex <==
\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{3pt}
\scriptsize % Reduce the font size for the table
\caption{Avg. distance to k-nearest prototypes across items by popularity. ProtoMF trained on LastFM-2b dataset with 80 prototypes. Distance is $1 - \text{sim}(i, p)$ between item $i$ and prototype $p$.}
\begin{tabular}{c | c c c}
\hline
\textbf{k} & \textbf{Least 25\%} & \textbf{25\%-50\%} & \textbf{Top 1\%} \\ \hline
1  & 0.35 & 0.32 & 0.30 \\ 
20 & 0.55 & 0.50 & 0.45 \\ 
40 & 0.70 & 0.65 & 0.60 \\ 
60 & 0.82 & 0.77 & 0.73 \\ 
80 & 0.93 & 0.90 & 0.88 \\ \hline
\end{tabular}
\label{tab:prototype_distances}
\end{table}

\begin{table}[h!]
\centering
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{10pt}
\caption{Average distance to k-nearest prototypes across items with different popularity levels. The ProtoMF model is trained on the LastFM-2b dataset with 80 prototypes. The distance is calculated as $1 - \text{sim}(i, p)$, where $i \in \mathbb{R}^{d}$ represents an item, and $p \in \mathbb{R}^{d}$ represents a prototype.}
\begin{tabular}{c | c c c}
\hline
\textbf{Number of Neighbors (k)} & \textbf{Least Popular 25\% Items} & \textbf{25\% to 50\% Least Popular Items} & \textbf{Top 1\% Most Popular Items} \\ \hline
1  & 0.35 & 0.32 & 0.30 \\ 
20 & 0.55 & 0.50 & 0.45 \\ 
40 & 0.70 & 0.65 & 0.60 \\ 
60 & 0.82 & 0.77 & 0.73 \\ 
80 & 0.93 & 0.90 & 0.88 \\ \hline
\end{tabular}
\label{tab:prototype_distances}
\end{table}


